Computing Area-Optimal Simple Polygonizations

We consider methods for finding a simple polygon of minimum (Min-Area) or maximum (Max-Area) possible area for a given set of points in the plane. Both problems are known to be NP-hard; at the center of the recent CG Challenge, practical methods have received considerable attention. However, previous methods focused on heuristic methods, with no proof of optimality. We develop exact methods, based on a combination of geometry and integer programming. As a result, we are able to solve instances of up to n=25 points to provable optimality. While this extends the range of solvable instances by a considerable amount, it also illustrates the practical difficulty of both problem variants.

==> grid_empty_grid_full.tex <==
\begin{subfigure}[b]{.5\textwidth}
\centering
\begin{tikzpicture}[line cap=round,line join=round,>=stealth,x=1cm,y=1cm]
\foreach \x in {-3,...,3}
    \foreach \y in {-3,...,3}
    {
    \fill (\x,\y) circle (1pt);
    }

\fill (0,0) circle (2pt);
\fill (0,1) circle (2pt);
\fill (0,2) circle (2pt);
\fill (1,0) circle (2pt);
\fill (2,-1) circle (2pt);
\fill (3,-2) circle (2pt);
\fill (1,-1) circle (2pt);
\fill (0,-1) circle (2pt);
\fill (-1,-1) circle (2pt);
\fill (-2,-1) circle (2pt);
\end{tikzpicture}

\caption{Point set with integer coordinates}

\end{subfigure}\begin{subfigure}[b]{.5\textwidth}
\centering
\begin{tikzpicture}[line cap=round,line join=round,>=stealth,x=1cm,y=1cm]
\foreach \x in {-3,...,3}
    \foreach \y in {-3,...,3}
    {
    \fill (\x,\y) circle (1pt);
    }

\fill (0,0) circle (2pt);
\fill (0,1) circle (2pt);
\fill (0,2) circle (2pt);
\fill (1,0) circle (2pt);
\fill (2,-1) circle (2pt);
\fill (3,-2) circle (2pt);
\fill (1,-1) circle (2pt);
\fill (0,-1) circle (2pt);
\fill (-1,-1) circle (2pt);
\fill (-2,-1) circle (2pt);

\draw[] (0,0)--(0,1) -- (0,2) -- (1,0) -- (2,-1) -- (3,-2) -- (1,-1) -- (0,-1) -- (-1, -1) -- (-2, -1) -- cycle;


\end{tikzpicture}

\caption{\textsc{Grid Empty} polygonization}

\end{subfigure}


==> short-03.tex <==
\section{Tools}
\label{sec:tools}
We considered two models based on integer programming: an \emph{edge-based formulation}
(described in Section~\ref{sec:edge}) and a \emph{triangle-based formulation}
(described in Section~\ref{sec:triangle}). In addition, we developed a number
of further refinements and improvements (described in Section~\ref{sec:enhance}).

\subsection{Edge-Based Formulation}
\label{sec:edge}
The first formulation is based on considering \emph{directed} edges of the polygon boundary. 
As shown in Figure~\ref{fig:reference_point_approach:area_calculation},
the area $A_{\cal P}$ of a polygon $\cal P$ can be computed by adding the (signed) triangle areas $f_e$
that are formed by edges $e$ and an arbitrary, fixed reference point $r$.

\begin{figure}[h]
\centering
\begin{subfigure}[b]{.5\textwidth}
\centering
\input{figures/reference_point_approach_polygon_triangles}%
\caption{Triangles of the polygon}
\label{fig:reference_point_approach:polygon_triangles}
\end{subfigure}%
\begin{subfigure}[b]{.5\textwidth}
\centering
\input{figures/reference_point_approach_polygon_triangles_positive}%
\caption{Positive edge triangles}
\label{fig:reference_point_approach:polygon_positive}
\end{subfigure}%

\begin{subfigure}[b]{.5\textwidth}
\centering
\input{figures/reference_point_approach_polygon_triangles_negative}%
\caption{Negative edge triangles}
\label{fig:reference_point_approach:polygon_negative}
\end{subfigure}\begin{subfigure}[b]{.5\textwidth}
\centering
\input{figures/reference_point_approach_polygon_triangles_sum}%
\caption{Calculated difference between (b) and (c)}
\label{fig:reference_point_approach:polygon_area}
\end{subfigure}
\caption[Area computation according to the edge-based approach]{Area computation of a polygon using a reference point $r$}
\label{fig:reference_point_approach:area_calculation}
\end{figure}

This leads to the following IP formulation, where the \emph{slab inequalities}~(\ref{ip:reference_point_approach:slabs}) ensure
that the polygon has a counterclockwise orientation, while (\ref{ip:reference_point_approach:subtours}) are \emph{subtour constraints}.

\begin{equation}
  \{\min , \max\} \sum_{e^+ \in E^r} z_{e^+} \cdot f_e - \sum_{e^- \in E^r} z_{e^-} \cdot f_e \label{ip:reference_point_approach:objective}\\
\end{equation}
\begin{align}
\vphantom{\sum_{i=1}^{m}} \forall s_i \in S: \qquad& \sum_{(j,i) \in \delta^+(s_i)} z_{ji} = 1 \label{ip:reference_point_approach:in_degree}\\
\vphantom{\sum_{i=1}^{m}} \forall s_i \in S: \qquad& \sum_{(i,j) \in \delta^-(s_i)} z_{ij} = 1 \label{ip:reference_point_approach:out_degree}\\
\vphantom{\sum_{i=1}^{m}} \forall e=\{i,j\} \in E: \qquad& z_{ij} + z_{ji} \leq 1 \label{ip:reference_point_approach:one_of_edges}\\
\vphantom{\sum_{i=1}^{m}} \forall \text{ intersecting}\quad \{i,j\}, \{k,l\} \in E: \qquad& z_{ij} + z_{ji} + z_{kl} + z_{lk} \leq 1 \label{ip:reference_point_approach:intersections}\\
\vphantom{\sum_{i=1}^{m}} (\forall \text{ slabs}\quad D) (\forall m=1,\ldots,\vert D \vert): \qquad& \sum_{i=1}^{m} z_{e_{i_D}^{lr}}-z_{e_{i_D}^{rl}} \label{ip:reference_point_approach:slabs}\\
\vphantom{\sum_{i=1}^{m}} \forall \emptyset \neq D \subsetneq S: \qquad& \begin{array}{l}\sum_{(k,l) \in \delta^-(D)} z_{kl} \geq 1 \\ \sum_{(k,l) \in \delta^+(D)} z_{kl} \geq 1\end{array}  \label{ip:reference_point_approach:subtours}\\
\forall e \in E^+ \mathrel{\dot\cup} E^-: \qquad& e \in \{0,1\}
\end{align}

As there are $\Theta(n^2)$ possible edges, the number of intersection constraints may be as big as $\Theta(n^4)$. Moreover,
the number of subtour constraints~(\ref{ip:reference_point_approach:subtours}) may be exponential, so they are only added
when necessary in an incremental fashion.

\subsection{Triangle-Based Formulation}
\label{sec:triangle}

An alternative is the {triangle-based formulation}, which considers the set $T(P)$ of
possibly $\binom{n}{3}$ many empty triangles of a point set $P$; see Figure~\ref{fig:triangulation_approach:max_triangles}
for an illustration. Making use of the fact that a simple polygon with $n$ vertices consists of $(n-2)$ empty
triangles with non-intersection interiors, we get the following IP formulation.

\begin{figure}[h]
\centering
  \input{figures/triangulation_approach_max_triangles}
  \caption[Empty triangle amount bound]{A set of five points and its ten empty triangles.}
  \label{fig:triangulation_approach:max_triangles}
\end{figure}

\begin{equation}
  \{\min , \max\} \sum_{\subscripttriangle \in T} f_\subscripttriangle \cdot x_\subscripttriangle \label{ip:triangulation_approach:objective}\\
\end{equation}
\begin{align}
\vphantom{\sum_{i=1}^{n}} \qquad& \sum_{\subscripttriangle \in T} x_\subscripttriangle = n-2 \label{ip:triangulation_approach:triangle_count}\\
\vphantom{\sum_{i=1}^{n}} \forall s_i \in S: \qquad& \sum_{\subscripttriangle \in \delta(s_i)} x_\subscripttriangle \geq 1 \label{ip:triangulation_approach:in_each_point}\\
\vphantom{\sum_{i=1}^{m}} \forall \text{intersecting}\quad \triangle_i, \triangle_j \in T: \qquad& x_{\subscripttriangle_i} + x_{\subscripttriangle_j} \leq 1 \label{ip:triangulation_approach:intersections}\\
\vphantom{\sum_{i=1}^{n}} \forall \emptyset \neq D \subsetneq T, \vert D \vert \leq n-3: \qquad& \sum_{\subscripttriangle \in D} x_\subscripttriangle \leq \sum_{\subscripttriangle \in \delta(D)} x_\subscripttriangle + \vert D \vert - 1 \label{ip:triangulation_approach:subtours}\\
\vphantom{\sum_{i=1}^{n}} \forall \triangle \in T: \qquad& x_\subscripttriangle \in \{0,1\}
\end{align}

As there are $\Theta(n^3)$ possible empty triangles, the number of intersection constraints may be as big as $\Theta(n^6)$. Again,
the number of subtour constraints~(\ref{ip:triangulation_approach:subtours}) may be exponential, so they are only added
when necessary in an incremental fashion.

\subsection{Enhancing the Integer Programs}
\label{sec:enhance}

Given the considerable size of the described IP formulations, we employed a number of enhancements to improve efficiency.
%due to limited space, we only give very brief sketches.
For points on the \textbf{convex hull}, only a reduced number of neighbors need to be considered.
Employing good \textbf{initial solutions} improves the performance in branch-and-bound searching;
we used a number of greedy heuristics, as well as the $\frac{1}{2}$-approximation of Fekete.
The large number of corresponding inequalities made it particularly important to deal with \textbf{intersections}
in an efficient manner: we condensed the constraints for cliques of intersecting objects into single
inequalities, and introduced special \emph{halfspace inequalities} for the triangle-based approach.
Further increases in efficiency were obtained by careful choices of how to \textbf{branch on variables}
and careful maintenance of \textbf{subtour constraints}.



==> solvers.tex <==
\begin{comment}
\begin{itemize}
\item BoundaryV1 (EV1)
\begin{itemize}
  \item Circle Subtour constraints (Lazy)
  \item Intersections Before Execution
\end{itemize}

\item BoundaryV2 (EV3)
\begin{itemize}
  \item Branch Callback (intersections)
  \item Lazy Constraint Connected Components
  \item Lazy Constraint Clique Intersections
\end{itemize}

\item BoundaryV4 (EV4)
\begin{itemize}
  \item Branch Callback (intersections)
  \item Lazy Constraint Connected Components
  \item Lazy Constraint Clique Intersections
  \item Lazy Constraint Slab constraints
  \item User Cut Connected Components (Threshold)
\end{itemize}

\item BoundaryV5 (EV2)
\begin{itemize}
  \item Lazy Constraint Connected Components
  \item Lazy Constraint Clique Intersections
\end{itemize}
\end{itemize}
\end{comment}

\begin{comment}
  \begin{itemize}
  \item TriangleV1
  \begin{itemize}
    %\item Branch Callback Intersections
    \item Lazy Constraint Clique Intersections
    \item Lazy Constraint Avoid Connected Components
  \end{itemize}

  \item TriangleV2
  \begin{itemize}
    %\item Branch Callback Intersections
    \item Lazy Constraint Clique Intersections
    \item Lazy Constraint Avoid Connected Components
    \item Lazy Constraint Triangle Fan Expressions
  \end{itemize}

  \item TriangleV3
  \begin{itemize}
    %\item Branch Callback Intersections
    \item Lazy Constraint Clique Intersections
    \item Lazy Constraint Avoid Connected Components
    \item Lazy Constraint Avoid Connected Point Components
    \item Lazy Constraint Triangle Fan Expressions
  \end{itemize}
\end{itemize}
\end{comment}

